Multi-Camera Industrial Open-Set Person Re-Identification and Tracking

In recent years, the development of deep learning approaches for the task of person re-identification led to impressive results. However, this comes with a limitation for industrial and practical real-world applications. Firstly, most of the existing works operate on closed-world scenarios, in which the people to re-identify (probes) are compared to a closed-set (gallery). Real-world scenarios often are open-set problems in which the gallery is not known a priori, but the number of open-set approaches in the literature is significantly lower. Secondly, challenges such as multi-camera setups, occlusions, real-time requirements, etc., further constrain the applicability of off-the-shelf methods. This work presents MICRO-TRACK, a Modular Industrial multi-Camera Re_identification and Open-set Tracking system that is real-time, scalable, and easy to integrate into existing industrial surveillance scenarios. Furthermore, we release a novel Re-ID and tracking dataset acquired in an industrial manufacturing facility, dubbed Facility-ReID, consisting of 18-minute videos captured by 8 surveillance cameras.

==> algo.tex <==

\begin{algorithm}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\caption{An algorithm with caption}\label{alg:cap}
\begin{algorithmic}
\Require \\ 
$model$ = re-identification model\\
$gallery$ = the open-set gallery\\
$frame$ = image of the current frame of video\\
$bboxes$ = list of detections coming from the tracker as tuple (track\_id, bbox, score)\\
$associations$ = dictionary with associations between $id_{tracker}$ and $id_{reid}$ for the current camera\\
$th_{score}$ = threshold for image quality\\
$th_{emb}$ = threshold for embedding distances
\Ensure list of individual IDs

\State // Compute the embedding of the people tracked. For each person, the person identifier is recovered from the gallery.

\State $idList \gets []$
\State $embeddingList \gets []$

\State $centroids \gets gallery.getCentroids()$ 

\For{$bbox$ in $bboxes$}
\State $reid \gets$ None
\State $embedding \gets$ None

\If {$bbox.score < th_{score}$}
\State continue
\EndIf
\State $probeEmb \gets model.inference(image, bbox)$ \Comment{Get current person embedding}
\State $reid \gets gallery.find(probeEmb, th_{emb})$ \Comment{If distance is $<$ than $th_{emb}$, None is returned}
\If {$reid \neq$ None}
\State $embedding \gets probeEmb$ 
\EndIf

\If {$bbox.track\_id \in associations$}
\State $reid \gets associations[bbox.track\_id]$
\EndIf
\State $embeddingList.add((reid, embedding, bbox.track\_id))$

\EndFor
\State // Get the centroids from the gallery. Initally the gallery is empty \Comment{Step 1}


\end{algorithmic}
\end{algorithm}

